Where did you get that? Towards Summarization Attribution for Analysts

Analysts require attribution, as nothing can be reported without knowing the source of the information. In this paper, we will focus on automatic methods for attribution, linking each sentence in the summary to a portion of the source text, which may be in one or more documents. We explore using a hybrid summarization, i.e., an automatic paraphrase of an extractive summary, to ease attribution. We also use a custom topology to identify the proportion of different categories of attribution-related errors.

==> AnnotationGuidelines/FACTS/overview-data.tex <==
This evaluation will use the CrisisFACTS data set. The data set consists of content snippets (approximately a sentence in length) from three content streams (Twitter, Reddit, online news sources) related to multiple crises (wildfires, hurricanes, floods). A summary is based on important facts for a day of a crisis event.

==> AnnotationGuidelines/FACTS/task1-examples.tex <==
\subsection*{Examples}
The upcoming examples are from fictitious content snippets (in the style of news and Twitter) related to crises during \textit{The Wonderful Wizard of Oz}. The examples are based on the original book.

\subsubsection*{Example: Support, Refute=no}
\mysample{
[SUMMARY] A cyclone dropped a house on the Wicked Witch of the East and killed her.\newline

[**EVAL**] Cyclone drops house on Wicked Witch of East \#cyclone \#eastwitch
}

The sentence to evaluate for attribution is “Cyclone drops house on Wicked Witch of East \#cyclone \#eastwitch”. This sentence provides supporting evidence for a cyclone dropping a house on the Wicked Witch of the East.
The summary statement is not fully supported since no evidence is provided for the Wicked Witch of the East being killed. However, partial support meets the definition of support.  You may mark “support” for an answer.

Consider the refute question next. The attribution sentence does not contain contradictory information. The answer is ``refute=no.''

\subsubsection*{Example: No Support, Refute=yes}
\mysample{
[SUMMARY] A scarecrow was stuck on a pole in the middle of a river after a rafting incident, and was saved by a child, a tin man, a lion, and a small animal of unknown origin.\newline

[**EVAL**] A scarecrow stuck on a pole in the middle of a cornfield was rescued by an unknown good samaritan. 
}

The attribution sentence does not provide supporting evidence for a river rescue because it describes a cornfield rescue. This example may be marked “no support”.

Consider the refute question next. While the attribution sentence describes a scarecrow rescue, this example will be marked as ``refute=yes'' because the type of rescue (cornfield versus river) differs.

This example could have also been marked as ``refute=no'' because the rescues differ too much to be related. There will be ambiguous cases like this where it is not clear if an attribution refutes a statement or not. We want you to use your best judgment during the evaluation.

If it helps to decide if a sentence refutes the summary statement or not, the purpose of the “refute” choice is to identify more focused algorithmic misfires. For example, when an automatic summarization method generates an incorrect fact (“hallucination”) like substituting one nationality over another (e.g., Winkies identified as Munchkins), or misinterprets the source document during text generation (e.g., child saves scarecrow misinterpreted as scarecrow saves child). Or when an attribution method provides a link which is related to the summary statement but misses the mark (e.g., cornfield rescue versus river rescue).

Another type of misfire is when the attribution method has low accuracy and picks an irrelevant sentence. We would like to capture this with “refute=no”.

\subsubsection*{Example: No Support, Refute=no}
\mysample{
[SUMMARY] A sleeping lion was rescued from a deadly poppy field by a large group of field mice, aided by a tin man, scarecrow, child, and an animal of unknown origin.\newline

[**EVAL**] WARNING: Large spider approaching. Seek shelter immediately! \#giantspider
}

There will be a topic-based relationship between a statement and an attribution. CrisisFACTS content snippets will be based on the same crises event. The examples in this document are based on crises from a single book, \textit{The Wonderful Wizard of Oz}. However, the connection is too tenuous for this example (lion rescue, spider attack), and it should be marked “no support”.


==> AnnotationGuidelines/FACTS/task2-examples.tex <==
\subsection*{Examples}
The upcoming examples are from fictitious content snippets (in the style of news and Twitter) related to crises during \textit{The Wonderful Wizard of Oz}. The examples are based on the original book.

\subsubsection*{Example: Full Support, Refute=no}
\mysample{
[SUMMARY] Winged Monkeys are feared due to frightful attacks, and are believed to be aligned with the Wicked Witch of the West.\newline

[**EVAL**] Winged Monkeys drop tin man from great heights to rocks below \#oznews\newline
[**EVAL**] Winged Monkeys tear out straw from scarecrow and leave clothes in tall tree. \#oznews\newline
[**EVAL**] Winged Monkeys kidnap child and small animal of unknown origin, imprison them in castle of Wicked Witch of West. \#oznews
}

You should consider all 3 sentences as part of the attribution for this task. The sentences in combination provide supporting evidence for multiple attacks by Winged Monkeys. The third sentence implies an affiliation between Winged Monkeys and the Wicked Witch of the West. The sentences fully support a statement that Winged Monkeys conduct fearful attacks and are aligned with the Wicked Witch of the West. This example can be marked “full support”.

Consider the refute question next. The three sentences support the summary statement and do not contain contradictory information. The answer is “refute=no”.



\subsubsection*{Example: Full support, Refute=no}
\mysample{
[SUMMARY] A cyclone dropped a house on the Wicked Witch of the East and killed her.\newline

[**EVAL**] The Wicked Witch of the East died due to injuries from a home dropped by a cyclone.\newline
[**EVAL**] Cyclone drops house on Wicked Witch of East \#cyclone \#eastwitch\newline
[**EVAL**] WARNING: tin man with sharp axe in area, attacked Tree Border Patrol. Considered very dangerous. Do not approach! \#livingforest
}

The first sentence fully supports the summary statement. The second sentence partially supports the statement. The third sentence is not related to this accident. While the third sentence does not provide supporting evidence, the three sentences when viewed as a group provide full support, and this example can be marked “full support”.

Consider the refute question next. The first two sentences support the summary statement and do not contain contradictory information. The third sentence is irrelevant. An irrelevant sentence is not a refutation. The answer is “refute=no”.

\subsubsection*{Example: Partial support, Refute=no}
\mysample{
[SUMMARY] The Wicked Witch of the West is aligned with Wolves, Crows, and Munchkins, who further her political agenda through acts which induce fear.\newline

[**EVAL**] Oz News Exclusive: Wicked Witch of West pays Wolves, Crows, and Black Bees to terrify populace. \#oznews\newline
[**EVAL**] Wolves attack and kill protesters outside of Wicked Witch of the West’s castle \#oznews\newline
[**EVAL**] WARNING: Crows approach. Seek shelter immediately! \#oznews \#landofthewest
}

The first two sentences provide supporting evidence that Wolves and Crows are aligned with the Wicked Witch of the West and use fear-based methods on her behalf. The third statement provides additional information that crows are viewed as dangerous in the Land of the West.  None of the sentences support an alliance with Munchkins. Mark this example as “partial support” since the sentences partially support the summary. 

The detail about Munchkins is a mistake in the summary. Munchkins are a peaceful people living in a region controlled by the Wicked Witch of the East, and are not agents of terror.  Full support will not be possible due to the mistake in the summary.

Consider the “refute” question next. None of the attribution sentences contain information that refute the summary statement. The answer may be marked “refute=no”. 

\subsubsection*{Example: No Support, Refute=yes}
\mysample{
[SUMMARY] The King of the Winged Monkeys thanked the Good Witch of the South for freeing them from magical cap enslavement, and declared that they would return to the Great Forest.\newline

[**EVAL**] Dorothy thanked the Good Witch of the South for telling her about the magical silver shoes and used them to return to Kansas.
[**EVAL**] China cow breaks leg after startled by giants. \#oznews \#daintychina\newline
[**EVAL**] Insure your home with Oz Insurance. \#ozinsurance
}

The 3 attribution sentences do not provide supporting evidence for the summary statement about Winged Monkeys. This example may be marked “no support”. 

Consider the refute question next. The summary statement and first attribution sentence are about two different cases where the Good Witch was thanked for magic-related repatriations (Winged Monkeys/magical cap versus Dororthy/magical shoes). This sentence will be treated as a refutation because it is related but different. The last two sentences are irrelevant and are not viewed as refutations.
Since there is one attribution sentence that refutes the summary statement, the question may be marked “refute=yes”.

This example could have also been marked as “refute=no” if you decided that the first sentence differed too much from the summary statement. There will be ambiguous cases like this where it is not clear if an attribution sentence is a refutation or not. We want you to use  your best judgment during the evaluation. 

If it helps to decide if a sentence refutes the summary statement or not, the
purpose of the “refute” choice is to identify more focused algorithmic misfires. For example, when an automatic summarization method generates an incorrect fact (“hallucination”) like substituting one nationality over another (e.g., Winkies identified as Munchkins), or misinterprets the source document during text generation (e.g., Dorothy thanks Good Witch misinterpreted as Good Witch thanks Dorothy). Or when an attribution method provides a link which is related to the summary statement but misses the mark (e.g., magical cap versus magical shoes).

Another type of misfire is when the attribution method has low accuracy and
picks an irrelevant sentence. We would like to capture this with “refute=no”

==> AnnotationGuidelines/Shared/preliminaries.tex <==
\section*{Preliminaries}
\textcolor{red}{@aaron - THIS SECTION IS FOR YOU TO PROVIDE INFINITYPOOL GUIDANCE}


==> AnnotationGuidelines/Shared/task1-nocontext.tex <==
\section*{Task 1: Judging the quality of a single attribution}
In this part, you will be provided a statement from the summary, and will be asked to judge the quality of a corresponding attribution in the source material. The statement will be a single sentence from the summary. The attribution will be a single (1) sentence from the source document.

Carefully read the summary statement and the attribution sentence with the surrounding context. The summary statement may appear to be very fluent and well-formed, and there may be slight differences compared to the corresponding attribution in the source document that is not easy to discern at first glance. Please pay close attention to the text, as if you were proofreading.

Your task will be to determine which category applies:
\begin{itemize}
\item \textbf{Support}: Some or all of the information in the summary statement is supported by the attribution sentence.
\item \textbf{No Support}: The attribution sentence does not support the summary statement. 
\item \textbf{Unclear (Can’t Make Judgement)}: The information provided does not make it possible to determine whether the attribution sentence supports or does not support the summary statement. The information is unclear, incomprehensible, malformed, or deficient in some other way.
\end{itemize}

The second part of the task will be to determine if the answer is ``yes'' or ``no'' to the following question:
\begin{itemize}
\item \textbf{Refute}: Does the  attribution contain information that refutes the summary statement? There can be a refutation (“yes”) with “support” or “no support”. Answer “no” if the information is unclear.
\end{itemize}


==> AnnotationGuidelines/facts-task1.tex <==
%%\documentclass[12pt]{article}
%%\usepackage{graphicx} % Required for inserting images
%%\usepackage{xcolor}
%%\usepackage[margin=1.25in]{geometry}

\newcommand{\mysample}[1]{
\begin{center}
\begin{minipage}{.80\textwidth}\fontfamily{lmss}\selectfont
#1
\end{minipage}
\end{center}
}


%%\title{Annotation Guidelines}
%%\author{CrisisFACTS}
%%\date{}

%%\begin{document}

%%\maketitle

\input{AnnotationGuidelines/Shared/overview}
\input{AnnotationGuidelines/FACTS/overview-data}

%\input{Shared/preliminaries}

\input{AnnotationGuidelines/Shared/task1-nocontext}
\input{AnnotationGuidelines/FACTS/task1-examples}

%\input{Shared/task2}
%\input{FACTS/task2-examples}

\input{AnnotationGuidelines/Shared/feedback}

%%\end{document}


==> AnnotationGuidelines/facts-task2.tex <==
%%\documentclass[12pt]{article}
%%\usepackage{graphicx} % Required for inserting images
%%\usepackage{xcolor}
%%\usepackage[margin=1.25in]{geometry}

\newcommand{\mysample}[1]{
\begin{center}
\begin{minipage}{.80\textwidth}\fontfamily{lmss}\selectfont
#1
\end{minipage}
\end{center}
}


%%\title{Annotation Guidelines}
%%\author{CrisisFACTS}
%%\date{}

%%\begin{document}

%%\maketitle

\input{AnnotationGuidelines/Shared/overview}
\input{AnnotationGuidelines/FACTS/overview-data}

%\input{Shared/preliminaries}

%\input{Shared/task1-nocontext}
%\input{FACTS/task1-examples}

\input{AnnotationGuidelines/Shared/task2}
\input{AnnotationGuidelines/FACTS/task2-examples}

\input{AnnotationGuidelines/Shared/feedback}

%%\end{document}


==> Definitions/journalnames.tex <==
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{scads}
{\gdef\@journal{scads}\gdef\@journalfull{Summer Conference on Applied Data Science (SCADS)}\gdef\@journalshort{SCADS}\gdef\@continuouspages{yes}}

==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/FACTS/overview-data.tex <==
This evaluation will use the CrisisFACTS data set. The data set consists of content snippets (approximately a sentence in length) from three content streams (Twitter, Reddit, online news sources) related to multiple crises (wildfires, hurricanes, floods). A summary is based on important facts for a day of a crisis event.

==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/FACTS/task1-examples.tex <==
\subsection*{Examples}
The upcoming examples are from fictitious content snippets (in the style of news and Twitter) related to crises during \textit{The Wonderful Wizard of Oz}. The examples are based on the original book.

\subsubsection*{Example: Support, Refute=no}
\mysample{
[SUMMARY] A cyclone dropped a house on the Wicked Witch of the East and killed her.\newline

[**EVAL**] Cyclone drops house on Wicked Witch of East \#cyclone \#eastwitch
}

The sentence to evaluate for attribution is “Cyclone drops house on Wicked Witch of East \#cyclone \#eastwitch”. This sentence provides supporting evidence for a cyclone dropping a house on the Wicked Witch of the East.
The summary statement is not fully supported since no evidence is provided for the Wicked Witch of the East being killed. However, partial support meets the definition of support.  You may mark “support” for an answer.

Consider the refute question next. The attribution sentence does not contain contradictory information. The answer is ``refute=no.''

\subsubsection*{Example: No Support, Refute=yes}
\mysample{
[SUMMARY] A scarecrow was stuck on a pole in the middle of a river after a rafting incident, and was saved by a child, a tin man, a lion, and a small animal of unknown origin.\newline

[**EVAL**] A scarecrow stuck on a pole in the middle of a cornfield was rescued by an unknown good samaritan. 
}

The attribution sentence does not provide supporting evidence for a river rescue because it describes a cornfield rescue. This example may be marked “no support”.

Consider the refute question next. While the attribution sentence describes a scarecrow rescue, this example will be marked as ``refute=yes'' because the type of rescue (cornfield versus river) differs.

This example could have also been marked as ``refute=no'' because the rescues differ too much to be related. There will be ambiguous cases like this where it is not clear if an attribution refutes a statement or not. We want you to use your best judgment during the evaluation.

If it helps to decide if a sentence refutes the summary statement or not, the purpose of the “refute” choice is to identify more focused algorithmic misfires. For example, when an automatic summarization method generates an incorrect fact (“hallucination”) like substituting one nationality over another (e.g., Winkies identified as Munchkins), or misinterprets the source document during text generation (e.g., child saves scarecrow misinterpreted as scarecrow saves child). Or when an attribution method provides a link which is related to the summary statement but misses the mark (e.g., cornfield rescue versus river rescue).

Another type of misfire is when the attribution method has low accuracy and picks an irrelevant sentence. We would like to capture this with “refute=no”.

\subsubsection*{Example: No Support, Refute=no}
\mysample{
[SUMMARY] A sleeping lion was rescued from a deadly poppy field by a large group of field mice, aided by a tin man, scarecrow, child, and an animal of unknown origin.\newline

[**EVAL**] WARNING: Large spider approaching. Seek shelter immediately! \#giantspider
}

There will be a topic-based relationship between a statement and an attribution. CrisisFACTS content snippets will be based on the same crises event. The examples in this document are based on crises from a single book, \textit{The Wonderful Wizard of Oz}. However, the connection is too tenuous for this example (lion rescue, spider attack), and it should be marked “no support”.


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/FACTS/task2-examples.tex <==
\subsection*{Examples}
The upcoming examples are from fictitious content snippets (in the style of news and Twitter) related to crises during \textit{The Wonderful Wizard of Oz}. The examples are based on the original book.

\subsubsection*{Example: Full Support, Refute=no}
\mysample{
[SUMMARY] Winged Monkeys are feared due to frightful attacks, and are believed to be aligned with the Wicked Witch of the West.\newline

[**EVAL**] Winged Monkeys drop tin man from great heights to rocks below \#oznews\newline
[**EVAL**] Winged Monkeys tear out straw from scarecrow and leave clothes in tall tree. \#oznews\newline
[**EVAL**] Winged Monkeys kidnap child and small animal of unknown origin, imprison them in castle of Wicked Witch of West. \#oznews
}

You should consider all 3 sentences as part of the attribution for this task. The sentences in combination provide supporting evidence for multiple attacks by Winged Monkeys. The third sentence implies an affiliation between Winged Monkeys and the Wicked Witch of the West. The sentences fully support a statement that Winged Monkeys conduct fearful attacks and are aligned with the Wicked Witch of the West. This example can be marked “full support”.

Consider the refute question next. The three sentences support the summary statement and do not contain contradictory information. The answer is “refute=no”.



\subsubsection*{Example: Full support, Refute=no}
\mysample{
[SUMMARY] A cyclone dropped a house on the Wicked Witch of the East and killed her.\newline

[**EVAL**] The Wicked Witch of the East died due to injuries from a home dropped by a cyclone.\newline
[**EVAL**] Cyclone drops house on Wicked Witch of East \#cyclone \#eastwitch\newline
[**EVAL**] WARNING: tin man with sharp axe in area, attacked Tree Border Patrol. Considered very dangerous. Do not approach! \#livingforest
}

The first sentence fully supports the summary statement. The second sentence partially supports the statement. The third sentence is not related to this accident. While the third sentence does not provide supporting evidence, the three sentences when viewed as a group provide full support, and this example can be marked “full support”.

Consider the refute question next. The first two sentences support the summary statement and do not contain contradictory information. The third sentence is irrelevant. An irrelevant sentence is not a refutation. The answer is “refute=no”.

\subsubsection*{Example: Partial support, Refute=no}
\mysample{
[SUMMARY] The Wicked Witch of the West is aligned with Wolves, Crows, and Munchkins, who further her political agenda through acts which induce fear.\newline

[**EVAL**] Oz News Exclusive: Wicked Witch of West pays Wolves, Crows, and Black Bees to terrify populace. \#oznews\newline
[**EVAL**] Wolves attack and kill protesters outside of Wicked Witch of the West’s castle \#oznews\newline
[**EVAL**] WARNING: Crows approach. Seek shelter immediately! \#oznews \#landofthewest
}

The first two sentences provide supporting evidence that Wolves and Crows are aligned with the Wicked Witch of the West and use fear-based methods on her behalf. The third statement provides additional information that crows are viewed as dangerous in the Land of the West.  None of the sentences support an alliance with Munchkins. Mark this example as “partial support” since the sentences partially support the summary. 

The detail about Munchkins is a mistake in the summary. Munchkins are a peaceful people living in a region controlled by the Wicked Witch of the East, and are not agents of terror.  Full support will not be possible due to the mistake in the summary.

Consider the “refute” question next. None of the attribution sentences contain information that refute the summary statement. The answer may be marked “refute=no”. 

\subsubsection*{Example: No Support, Refute=yes}
\mysample{
[SUMMARY] The King of the Winged Monkeys thanked the Good Witch of the South for freeing them from magical cap enslavement, and declared that they would return to the Great Forest.\newline

[**EVAL**] Dorothy thanked the Good Witch of the South for telling her about the magical silver shoes and used them to return to Kansas.
[**EVAL**] China cow breaks leg after startled by giants. \#oznews \#daintychina\newline
[**EVAL**] Insure your home with Oz Insurance. \#ozinsurance
}

The 3 attribution sentences do not provide supporting evidence for the summary statement about Winged Monkeys. This example may be marked “no support”. 

Consider the refute question next. The summary statement and first attribution sentence are about two different cases where the Good Witch was thanked for magic-related repatriations (Winged Monkeys/magical cap versus Dororthy/magical shoes). This sentence will be treated as a refutation because it is related but different. The last two sentences are irrelevant and are not viewed as refutations.
Since there is one attribution sentence that refutes the summary statement, the question may be marked “refute=yes”.

This example could have also been marked as “refute=no” if you decided that the first sentence differed too much from the summary statement. There will be ambiguous cases like this where it is not clear if an attribution sentence is a refutation or not. We want you to use  your best judgment during the evaluation. 

If it helps to decide if a sentence refutes the summary statement or not, the
purpose of the “refute” choice is to identify more focused algorithmic misfires. For example, when an automatic summarization method generates an incorrect fact (“hallucination”) like substituting one nationality over another (e.g., Winkies identified as Munchkins), or misinterprets the source document during text generation (e.g., Dorothy thanks Good Witch misinterpreted as Good Witch thanks Dorothy). Or when an attribution method provides a link which is related to the summary statement but misses the mark (e.g., magical cap versus magical shoes).

Another type of misfire is when the attribution method has low accuracy and
picks an irrelevant sentence. We would like to capture this with “refute=no”

==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/Shared/feedback.tex <==
\section*{Questions or Feedback?}
If you have questions about the task, or any feedback about how we could make it better or what your experience was like with it, please contact us on Slack using the channel \texttt{\#inf-attribution-evaluation} and we'll get back to you. Thanks!

==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/Shared/overview.tex <==
\section*{Overview}
We are a team interested in evaluating attribution for summarization (how to link automatically generated summaries back to their source material.)

In this project, you will evaluate the quality of attributions for summaries that have been created by humans or by automatic methods that mimic what humans would write. We would like to evaluate if an attribution method can provide accurate attributions, and if the accuracy is influenced by the type of automatic summarization method used.

At a high level, the project breaks down into two tasks:

\begin{enumerate}
    \item Given a statement in a summary, judge the quality of a single attribution.
    \item Given a statement in a summary, judge whether the statement is fully supported by three (ranked) attributions.
\end{enumerate}

Examples of the task you have chosen will be provided in this document.



==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/Shared/preliminaries.tex <==
\section*{Preliminaries}
\textcolor{red}{@aaron - THIS SECTION IS FOR YOU TO PROVIDE INFINITYPOOL GUIDANCE}


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/Shared/task1-context.tex <==
\section*{Task 1: Judge the quality of a single attribution}
In this part, you will be provided a statement from the summary, and will be asked to judge the quality of a corresponding attribution in the source material. The statement will be a single sentence from the summary. The attribution will be a single (1) sentence from the source document, along with surrounding context sentences (sentence before and sentence after the attribution sentence in the source document, if available).

Carefully read the summary statement and the attribution sentence with the surrounding context. The summary statement may appear to be very fluent and well-formed, and there may be slight differences compared to the corresponding attribution in the source document that is not easy to discern at first glance. Please pay close attention to the text, as if you were proofreading.

Your task will be to determine which category applies:
\begin{itemize}
\item \textbf{Support}: Some or all of the information in the summary statement is supported by the attribution sentence.
\item \textbf{No Support}: The attribution sentence does not support the summary statement. 
\item \textbf{Unclear (Can’t Make Judgement)}: The information provided does not make it possible to determine whether the attribution sentence supports or does not support the summary statement. The information is unclear, incomprehensible, malformed, or deficient in some other way.
\end{itemize}

The second part of the task will be to determine if the answer is ``yes'' or ``no'' to the following question:
\begin{itemize}
\item \textbf{Refute}: Does the attribution contain information that refutes the summary statement? There can be a refutation (``yes'') with ``support'' or ``no support''. Answer ``no'' if the information is unclear.
\end{itemize}

==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/Shared/task1-nocontext.tex <==
\section*{Task 1: Judging the quality of a single attribution}
In this part, you will be provided a statement from the summary, and will be asked to judge the quality of a corresponding attribution in the source material. The statement will be a single sentence from the summary. The attribution will be a single (1) sentence from the source document.

Carefully read the summary statement and the attribution sentence with the surrounding context. The summary statement may appear to be very fluent and well-formed, and there may be slight differences compared to the corresponding attribution in the source document that is not easy to discern at first glance. Please pay close attention to the text, as if you were proofreading.

Your task will be to determine which category applies:
\begin{itemize}
\item \textbf{Support}: Some or all of the information in the summary statement is supported by the attribution sentence.
\item \textbf{No Support}: The attribution sentence does not support the summary statement. 
\item \textbf{Unclear (Can’t Make Judgement)}: The information provided does not make it possible to determine whether the attribution sentence supports or does not support the summary statement. The information is unclear, incomprehensible, malformed, or deficient in some other way.
\end{itemize}

The second part of the task will be to determine if the answer is ``yes'' or ``no'' to the following question:
\begin{itemize}
\item \textbf{Refute}: Does the  attribution contain information that refutes the summary statement? There can be a refutation (“yes”) with “support” or “no support”. Answer “no” if the information is unclear.
\end{itemize}


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/Shared/task2.tex <==
\section*{Task 2: Judge the quality of a group of attributions}

In this part, you will be provided a statement from the summary, and will be asked to judge the amount of support by the attribution. The statement will be a single sentence from the summary. The attribution will be three (3) sentences from the source material.

Carefully read the summary statement and the 3 attribution sentences. The summary statement may appear to be very fluent and well-formed, and there may be slight differences compared to the corresponding 3 attribution sentences from the source data that is not easy to discern at first glance. Please pay close attention to the text, as if you were proofreading.

Your task will be to determine which category applies:
\begin{itemize}
\item \textbf{Full Support}: All of the information in the summary statement is supported by the attribution sentences.
\item \textbf{Partial Support}: Only some of the information in the summary statement is supported, but other parts of the information are missing.
\item \textbf{No Support}: The attribution sentences do not support the summary statement.  
\item \textbf{Unclear (Can't Make Judgment)}: The information provided does not make it possible to determine whether the attribution sentence fully supports, partially supports, or does not support the summary statement. The information is unclear, incomprehensible, malformed, or deficient in some other way. 
\end{itemize}

The second part of the task will be to determine if the answer is “yes” or “no” to the following question:
\begin{itemize}
\item \textbf{Refute}: Does the attribution contain information that refutes the summary statement? There can be a refutation (“yes”) with “full support”, “partial support”, or “no support”. Answer “no” if the information is unclear.
\end{itemize}

==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/TAC2011/overview-data.tex <==
 This evaluation will use the TAC 2011 (Text Analysis Conference) data set for multi-document summarization. The data set contains news articles grouped by topic (10 documents per topic). A summary is based on a single topic (10 documents).

==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/TAC2011/task1-examples.tex <==
\subsection*{Examples}

For TAC 2011, a summary is based on 10 documents for a single topic. The upcoming examples are from a single topic on threats to sea turtles.

\subsubsection*{Example: Support, Refute=no}
\mysample{
[SUMMARY] Sea turtles are threatened by increased poaching, habitat destruction for land development, illegal fishing, and pollution.\newline

[CONTEXT] The fishermen do not properly release the turtles and often kill them, leaving them to wash ashore. \newline
[**EVAL**] Turtles that come to lay eggs on the beaches may be killed by pollution, stray dogs or foxes, or captured by tourists. \newline
[CONTEXT] Mohammad Aminul Islam, the top administrator for the area, ordered local officials to teach people, from fishermen to tourists, to change their behavior.
}

The sentence to evaluate for attribution is “Turtles that come to lay eggs on the beaches may be killed by pollution, stray dogs or foxes, or captured by tourists.” This sentence provides supporting evidence that sea turtles are threatened by pollution. While the first context sentence supports illegal fishing, the decision for the evaluation should only be based on the sentence with the {\fontfamily{lmss}\selectfont[**EVAL**]} (evaluate) prefix.

The summary statement is not fully supported since no supporting evidence is provided for poaching, habitat destruction for land development, and illegal fishing by the attribution sentence. However, partial support meets the definition of support. You may mark “support” for an answer.

Consider the refute question next. The attribution sentence supports the summary statement and also contains supplemental information. It does not contain contradictory information. The answer is ``refute=no''.

\subsubsection*{Example: No Support, Refute=yes}
\mysample{
[SUMMARY] Malaysia has arrested a number of poachers, many from south China, for poaching turtles and other animals.\newline

[CONTEXT] At that price, a single nest containing about 100 eggs nets a poacher 1,000 pesos. Compare that, he says, to Mexico's minimum daily wage of 45 pesos. \newline
[**EVAL**] The Mexican government takes poaching seriously, he continued, assessing steep fines or jail time--``it's a worse offense than drugs''--but it lacks the manpower to prevent the crime in the first place or prosecute offenders in the second. \newline
[CONTEXT] Rapid development endangers the turtles. 
}

The attribution sentence is the second of three consecutive sentences. This sentence does not provide supporting evidence for poaching in Malaysia because the attribution is about poaching in Mexico which is a different country. (The difference is due to the summary being based on a different news article than the attribution.) You may mark ``no support.''

Consider the refute question next. While the attribution sentence supports turtle poaching having legal repercussions, this example will be marked as “refute=yes” because the country differs. 

This example could have also been marked as “refute=no” because the statement and attribution sentence are about different countries. There will be ambiguous cases like this where it is not clear if an attribution refutes a statement or not. We want you to use your best judgment during the evaluation. 

If it helps to decide between “refute=yes” and “refute=no”, the purpose of the “refute” choice is to identify more focused algorithmic misfires. For example, when an automatic summarization method generates an incorrect fact (“hallucination”) like substituting one nationality for another, or misinterprets the source document during text generation (e.g., dog bites man misinterpreted as man bites dog). Or when an attribution method provides a link which is related to the summary statement but misses the mark (e.g., Mexican poaching instead of Malaysian poaching).

Another type of misfire is when the attribution method has low accuracy and picks an irrelevant sentence. We would like to capture this with the “refute=no”.  

\subsubsection*{Example: No Support, Refute=no}
\mysample{
[SUMMARY] 90 sea turtles were rescued in Mexico when they became comatose from a cold snap.\newline

[CONTEXT] Some sea turtle species eat jellyfish like they are going out of style.\newline 
[**EVAL**] If the turtles weren't around to eat the jellyfish, the jellyfish population would explode.\newline 
[CONTEXT] The hungry jellyfish hordes would gorge on zooplankton.
}

The attribution sentence is “If the turtles weren't around to eat the jellyfish, the jellyfish population would explode.” This sentence does not provide supporting evidence for a turtle rescue. You may mark ``no support.''

 Consider the refute question. There will be a topic-based relationship between a statement and an attribution with TAC 2011 since the summary is based on news articles from the same topic (e.g., threats to sea turtles). However, the connection is too tenuous for this example, and it should be marked “refute=no”.


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/TAC2011/task2-examples.tex <==
\subsection*{Examples}

For TAC 2011, a summary is based on 10 documents for a single topic. The upcoming examples are from a single topic on threats to sea turtles.

\subsubsection*{Example: Full support, Refute=no}
\mysample{
[SUMMARY] Some countries have passed laws to protect the turtles.\newline

[**EVAL**] The Mexican government takes poaching seriously, he continued, assessing steep fines or jail time--``it's a worse offense than drugs''--but it lacks the manpower to prevent the crime in the first place or prosecute offenders in the second.\newline
[**EVAL**] A Malaysian court Friday jailed a group of 13 Chinese fishermen for 18 months each for poaching nearly 80 protected turtles.\newline
[**EVAL**] Ahmed would not give any specific reason for the spike in deaths, but said the use of illegal fishing nets near the shoreline has apparently increased recently.
}

%You should consider all 3 sentences as part of the attribution for Task 2 of the evaluation.
The first sentence describes a poaching law in Mexico. Malaysian law can be inferred by the second sentence. The third sentence describes illegal fishing nets but does not specify the country (Bangladesh). Combined, the sentences are sufficient to fully support a statement that more than one country has laws to protect turtles, and the example can be marked ``full support''.

Consider the refute question next. Each sentence supports the summary statement and does not contain contradictory information. The answer is ``refute=no''.

\subsubsection*{Full support, Refute=no}
\mysample{
[SUMMARY] 90 sea turtles were rescued in Mexico when they became comatose from a cold snap.\newline


[**EVAL**] Nearly 90 sea turtles rescued after a cold snap left them comatose have been returned to the Gulf of Mexico.\newline
[**EVAL**] Dozens of rehabilitated sea turtles, threatened by cold, returned to Gulf of Mexico.\newline
[**EVAL**] Green turtles are born in southern Mexico and spend their early years feeding on turtle grass in shallow areas such as the Laguna Madre.
}

The first sentence fully supports the summary statement. The second sentence partially supports the statement. The third sentence is about turtles in Mexico but not a rescue. %While the third sentence does not provide supporting evidence, the three sentences when viewed as a group provide full support, and this example can be marked “full support.” 
If one or two sentences fully support the summary statement, the question may be marked ``full support''. Support is not required  from all 3 sentences.

Consider the refute question next. The first two sentences support the summary sentence and do not contain contradictory information. The third sentence is about Mexican turtles but is about a different topic (rescue versus early life). The connection is tenuous and will not be viewed as a refutation. Since none of the sentences contain a refutation, the answer to the question is “refute=no”.

This example could have also been marked as “refute=yes” because the third sentence is about Mexican turtles so there is a connection between that sentence and the summary statement, but the facts are different. There will be ambiguous cases like this where it is not clear if an attribution sentence refutes a statement or not. We want you to use your best judgment during the evaluation.

If it helps to decide if a sentence refutes the summary statement or not, the purpose of the “refute” choice is to identify more focused algorithmic misfires. For example, when an automatic summarization method generates an incorrect fact (“hallucination”) like substituting one nationality over another, or misinterprets the source document during text generation (e.g., dog bites man misinterpreted as man bites dog). Or when an attribution method provides a link which is related to the summary statement but misses the mark.  

Another type of misfire is when the attribution method has low accuracy and picks an irrelevant sentence. We would like to capture this with ``refute=no''.

\subsubsection*{Full support, Refute=yes}
\mysample{
[SUMMARY] 17 Chinese nationals found with 274 protected turtles, most of them dead, were recently arrested in Malaysian waters.\newline

[**EVAL**] The poachers were caught by Malaysian marine police on March 28 in waters off the coast of eastern Sabah state with a catch of 274 protected Hawksbill and Green turtles, only 32 of which were still alive.\newline
[**EVAL**] They were the second group of fishermen from China's Hainan island jailed this week for turtle poaching off the waters of Malaysia's eastern Sabah state, with 17 men sentenced on Wednesday for catching 274 of the creatures.\newline
[**EVAL**] A Malaysian court Friday jailed a group of 13 Chinese fishermen for 18 months each for poaching nearly 80 protected turtles. 
}

The first sentence provides supporting evidence for poachers being caught with 274 protected turtles, most of them dead. The second sentence provides support for the arrest of 17 Chinese nationals with 274 turtles. The third sentence is about a different arrest.
The first two sentences provide full support for the summary statement, and this example may be marked ``full support''.

Consider the refute question next. The third sentence is on the same subject: a Malaysian arrest of Chinese nationals for poaching protected turtles. However, it is about a different arrest. This is an example of a misfire where a sentence is related but misses the mark, and can be viewed as an instance of ``refute=yes''.

\subsubsection*{Partial support, Refute=no}
\mysample{
[SUMMARY] Sea turtles are threatened by increased poaching, habitat destruction for land development, illegal fishing, and pollution.\newline

[**EVAL**]  The turtles--which can be found in other parts of Asia along the Andaman Coast and the South China Sea--have seen their numbers reduced drastically in recent years mostly due to poaching of their eggs, pollution and habitat loss.\newline
[**EVAL**] Turtles that come to lay eggs on the beaches may be killed by pollution, stray dogs or foxes, or captured by tourists.\newline
[**EVAL**] Sea turtles face a host of threats around the world. 
}

The three sentences provide supporting evidence for a threat to sea turtles for several reasons but do not support illegal fishing. This example may be marked “partial support”.

None of the sentences refute the summary sentence. The answer is “refute=no”.
 
\subsubsection*{Example: No support, Refute=no}
\mysample{
[SUMMARY] Scientists say that the loss of sea turtles could have unforeseen, even catastrophic, consequences.\newline

[**EVAL**] Efforts in Mexico to protect sea turtles are a patchwork of official and unofficial endeavors, according to Sea Turtle, Inc., a nonprofit based in South Padre Island.\newline
[**EVAL**] ``We are trying to mobilize resources to make a bigger plan to save the sea turtles in the future.''\newline
[**EVAL**] Thai villagers have caught a river terrapin turtle that was thought to be extinct in the country.
}

Sentences will be related to a common topic (threats to sea turtles). However, the 3 attribution sentences do not support the summary statement. This example may be marked “no support”. 

Consider the refute question next. Each attribution sentence is irrelevant to the summary statement. An irrelevant sentence is not a refutation. None of the sentences refute the summary statement and the question may be marked “refute=no”.


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/TAC2011/task2-faq.tex <==
\newcounter{question}
\setcounter{question}{0}

\newcommand{\question}[1]{\item[Q\refstepcounter{question}\thequestion.] #1}
\newcommand{\answer}[1]{\item[A\thequestion.] #1}

\subsubsection*{FAQ}
\begin{itemize}
\question\textit{How do we mark a group of attribution sentences if one of the sentences fully supports the summary statement, no matter what the rest say? Do we mark this as ``full support'' or ``partial support''?}
\answer If one attribution sentence fully supports the summary statement, then mark the group as ``full support'' for the first question.

\question\textit{In InfinityPool (the annotator platform), choices were not pre-selected for the first question about support. However, an answer was already highlighted for the second refute question before I answered it. Should this happen?}
\answer The refute questions all default to ``no''. Change an answer to ``yes'' (when applicable).
\end{itemize}


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/facts-task1.tex <==
%%\documentclass[12pt]{article}
%%\usepackage{graphicx} % Required for inserting images
%%\usepackage{xcolor}
%%\usepackage[margin=1.25in]{geometry}

\newcommand{\mysample}[1]{
\begin{center}
\begin{minipage}{.80\textwidth}\fontfamily{lmss}\selectfont
#1
\end{minipage}
\end{center}
}


%%\title{Annotation Guidelines}
%%\author{CrisisFACTS}
%%\date{}

%%\begin{document}

%%\maketitle

\input{AnnotationGuidelines/Shared/overview}
\input{AnnotationGuidelines/FACTS/overview-data}

%\input{Shared/preliminaries}

\input{AnnotationGuidelines/Shared/task1-nocontext}
\input{AnnotationGuidelines/FACTS/task1-examples}

%\input{Shared/task2}
%\input{FACTS/task2-examples}

\input{AnnotationGuidelines/Shared/feedback}

%%\end{document}


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/facts-task2.tex <==
%%\documentclass[12pt]{article}
%%\usepackage{graphicx} % Required for inserting images
%%\usepackage{xcolor}
%%\usepackage[margin=1.25in]{geometry}

\newcommand{\mysample}[1]{
\begin{center}
\begin{minipage}{.80\textwidth}\fontfamily{lmss}\selectfont
#1
\end{minipage}
\end{center}
}


%%\title{Annotation Guidelines}
%%\author{CrisisFACTS}
%%\date{}

%%\begin{document}

%%\maketitle

\input{AnnotationGuidelines/Shared/overview}
\input{AnnotationGuidelines/FACTS/overview-data}

%\input{Shared/preliminaries}

%\input{Shared/task1-nocontext}
%\input{FACTS/task1-examples}

\input{AnnotationGuidelines/Shared/task2}
\input{AnnotationGuidelines/FACTS/task2-examples}

\input{AnnotationGuidelines/Shared/feedback}

%%\end{document}


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/tac-task1.tex <==
%%\documentclass[12pt]{article}
%%\usepackage{graphicx} % Required for inserting images
%%\usepackage{xcolor}
%%\usepackage[margin=1.25in]{geometry}

\newcommand{\mysample}[1]{
\begin{center}
\begin{minipage}{.80\textwidth}\fontfamily{lmss}\selectfont
#1
\end{minipage}
\end{center}
}


%\title{Annotation Guidelines}
%\author{TAC 2011}
%\date{}

\maketitle

\input{AnnotationGuidelines/Shared/overview}
\input{AnnotationGuidelines/TAC2011/overview-data}

%\input{Shared/preliminaries}

\input{AnnotationGuidelines/Shared/task1-context}
\input{AnnotationGuidelines/TAC2011/task1-examples}

%\input{Shared/task2}
%\input{TAC2011/task2-examples}

\input{AnnotationGuidelines/Shared/feedback}

%%\end{document}


==> Human_Evaluation_Attribution_SCADS_2023/AnnotationGuidelines/tac-task2.tex <==
%%\documentclass[12pt]{article}
%%\usepackage{graphicx} % Required for inserting images
%%\usepackage{xcolor}
%%\usepackage[margin=1.25in]{geometry}

\newcommand{\mysample}[1]{
\begin{center}
\begin{minipage}{.80\textwidth}\fontfamily{lmss}\selectfont
#1
\end{minipage}
\end{center}
}


%%\title{Annotation Guidelines}
%%\author{TAC 2011}
%%\date{}

%%\begin{document}

%%\maketitle

\input{AnnotationGuidelines/Shared/overview}
\input{AnnotationGuidelines/TAC2011/overview-data}

%\input{Shared/preliminaries}

%\input{Shared/task1-context}
%\input{TAC2011/task1-examples}

\input{AnnotationGuidelines/Shared/task2}
\input{AnnotationGuidelines/TAC2011/task2-faq}
\input{AnnotationGuidelines/TAC2011/task2-examples}

\input{AnnotationGuidelines/Shared/feedback}

%%\end{document}


==> Human_Evaluation_Attribution_SCADS_2023/Definitions/journalnames.tex <==
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{scads}
{\gdef\@journal{scads}\gdef\@journalfull{Summer Conference on Applied Data Science (SCADS)}\gdef\@journalshort{SCADS}\gdef\@continuouspages{yes}}

==> Human_Evaluation_Attribution_SCADS_2023/RefutationAnalysis/refutation-analysis-tables.tex <==
%%% TAC 2011 HUMAN TASK 1 TABLE %%%
\begin{table}[p]\small
  \parbox[b]{4.85in}{}
  \centering
  \begin{tabular}{|l|c|c|c|p{1.5cm}|p{1cm}|p{4cm}|}
    \hline
    \textbf{ID} & \textbf{Method} & \textbf{Annotator} & \textbf{L} &
    \textbf{Primary} & \textbf{2nd} & \textbf{Comment} \\
    \hline
    13135 & Emb & 8d4ff & S &  Content  & OutE & Primary part of summary not present in attribution (=13245)\\ \hline
    % China environmental issue
    13181 & Emb & 8d4ff & N & Content & OutE & Summary contains information not present in attribution which is about a related topic \\ \hline
    % Walter Reed controversy
    13182 & Emb & 8f14c & U & Semantic & EntE & Time Shift led to inconsistent info (=13221)  \\ \hline
   % ferry sinking recovery efforts
   13189 & Emb & 8d4ff & S & Semantic Content & CircE OutE & Time Shift led to inconsistent timing info; Summary contains info not in attributing sentence but in context \\ \hline
   % liberian war crime trial
   13190 & Emb & 8d4ff & S & Content & OutE & Timing information in summary not present in attribution \\ \hline
   % Athens embassy attack
   \gray{13221} & \gray{Emb} & \gray{8d4ff} & \gray{S} & \gray{Semantic} & \gray{EntE} & \gray{Time Shift led to inconsistent info (=13182)} \\ \hline   % ferry sinking recovery efforts
   13229 & Emb & 8d4ff & S & Content & OutE & Timing info stated differently (August versus Thursday) \\ \hline
   % Mattel recall
   \gray{13245} & \gray{Emb} & \gray{8f14c} & \gray{U} & \gray{Content}  & \gray{OutE} & \gray{Primary part of summary not present in attribution (=13135)}\\ \hline
   % China environmental issue
   13258 & Emb & 8f14c & N & Content & OutE & Timing and supplemental location information in summary not present in attribution \\ \hline
   % piracy seizure
  \end{tabular}
  \parbox[b]{4.85in}{}
  \caption{TAC 2011: Human Summaries: Task 1: One Attributing Sentence with Context. L/Label: S=Support, N=No Support, U=Unclear.}
  \label{tab:human-task-1}
\end{table}

%%% TAC 2011 HUMAN TASK 2 TABLE %%%
\begin{table}[h]\small
  \parbox[b]{4.85in}{}
  \centering
  \begin{tabular}{|l|c|c|c|p{1.6cm}|p{1cm}|p{4.1cm}|}
    \hline
    \textbf{ID} & \textbf{Method} & \textbf{Annotator} & \textbf{L} &
    \textbf{Primary} & \textbf{2nd} & \textbf{Comment} \\
    \hline
    12981 & Emb & eed54 & P & Semantic & CircE & Time Shift error led to inconsistent timing info (2,3) \\ \hline
    % south korea oil tanker accident
    13022 & Emb & 415f6 & P & Content & OutE &  Summary contains statistic not present in attributions\\ \hline
    % china earthquake, stats (number dead) in news article but not in citations
    13025 & Emb & 415f6 & F & Content Additional & GramE OthE & Bad attribution grammar (2); Attribution on related topic (3)\\ \hline
    % internet redesign
    13039 & NLI & eed54 & F & Semantic & PredE  & Time Shift led to inconsistent info (3) (=13144)\\ \hline
    % Menu Foods recall
    13041 & NLI & 415f6 & F & Semantic & EntE & Attributions inconsistent but related (2,3) (=13046)\\ \hline
    % Arabs and shoe soles insult
    \gray{13046} & \gray{Emb} & \gray{415f6} & \gray{F} & \gray{Semantic} & \gray{EntE} & \gray{Attributions inconsistent but related (2,3) (=13041)}\\ \hline
    % Arabs and shoe soles insult
    13056 & NLI & 415f6 & F & Additional & OthE & Unrelated attribution (3)\\ \hline
    % construction and missing people
    13065 & Emb & 415f6 & F & Content & OutE &  Summary statement contains additional timing information not present in attributions\\ \hline
    % athens Embassy attack
    13072 & Emb & 415f6 & F & Semantic & PredE & Inconsistent info, from time shift or different disaster (3)\\ \hline
    % Bangledesh cyclone
    13095 & Emb & 415f6 & P & Content Additional & OutE OthE & Summary contains info not present in attributions; Attribution for wrong location (3)\\ \hline
    % SW China water shortage causes
    13097 & NLI & 415f6 & F & Additional & OthE  & Attribution unrelated (3)\\ \hline
    % bombing in India
    13098 & Emb & 415f6 & F & Additional & NE & Unclear why selected as refutation\\ \hline
    % construction and missing people, same summary, different citations 13056
    13104 & NLI & 415f6 & F & Additional & OthE & Attributions related (2,3) \\ \hline
    % madoff lawsuit
    13105 & Emb & 415f6 & F & Additional & OthE & Attributions related (2,3) \\ \hline
    % madoff lawsuit, same summary, diff citations 13104
    \gray{13144} & \gray{NLI} & \gray{415f6} & \gray{P} & \gray{Semantic} & \gray{PredE} & \gray{Time Shift led to inconsistent info (3) (=13039)}\\ \hline
    % menu foods, same summary, same citations 13039
  \end{tabular}
  \parbox[b]{4.85in}{}
  \caption{TAC 2011: Human Summaries: Task 2: Three Attributing Sentences. L/Label: F=Full Support, P=Partial Support.}
  \label{tab:tac2011-human-task2}
\end{table}


%%% TAC 2011 MACHINE TASK 2 %%%
\begin{table}[h]\small
  %\parbox[b]{4.85in}{}
  \centering
  \begin{tabular}{|l|c|c|c|p{1.6cm}|p{1.1cm}|p{4.1cm}|}
    \hline
    \textbf{ID} & \textbf{Method} & \textbf{Annot.} & \textbf{L} &
    \textbf{Primary} & \textbf{2nd} & \textbf{Comment} \\
    \hline
    13951 & Abstractive & 8d4ff & P & Content & OutE & Summary contains information not present in attributions but might be inferred\\ \hline
    % children trama-> inflammation and disease
    % summary about childhood impact, #2/#3 about adult disease from child trauma
    13954 & Abstractive & 8d4ff & P & Semantic Content & CircE OutE & Time shift (1,2); Summary contained info not present in attributions\\ \hline
    % Finnish PM expressed condolences, gov held emergency meeting
    13957 & Abstractive & 8d4ff & P & Semantic & PredE & Time shift led to inconsistent info (2,3) \\ \hline 
    % Cyclone disaster
    13961 & Abstractive & 8d4ff & F & Semantic & PredE & Time shift led to inconsistent info (3)\\ \hline
    % Minneapolis bridge collapse with fatalities
    13971 & Hybrid & 8d4ff & F & Content & OutE & Summary hallucination (1) (=14091)\\ \hline
    % Amish children killed
    % summary says "she had known for almost 10 years", source docs say married
    % to for almost 10 years
    \gray{14021} & \gray{Abstractive} & \gray{8f14c} & \gray{P} & \gray{Semantic} & \gray{PredE} & \gray{Time shift led to inconsistent info (3) (=13961, 14081)}\\ \hline
    % Minneapolis bridge collapse with fatalities
    14026 & Abstractive & 8f14c & F & Additional & OthE & Attribution contains related info (2)\\ \hline
    % Chinese FM offers conolences to air crash victims
    14045 & Hybrid & 8f14c & F & Semantic & PredE & Time shift led to inconsistent info (2) (=14105) \\ \hline
    % Iraqi reporter throws shoes at Pres Bush, one citation says shoe
    \gray{14077} & \gray{Abstractive} & \gray{36f2c} & \gray{P} & \gray{Semantic} & \gray{PredE} & \gray{Time shift led to inconsistent info (2,3) (=13597)}\\ \hline
    % Cyclone related: summary evacuation, citation homelessness
    \gray{14081} & \gray{Abstractive} & \gray{36f2c} & \gray{F} & \gray{Semantic} & \gray{PredE} & \gray{Time shift led to inconsistent info (3) (=13961,14021)}\\ \hline
    % Minneapolis bridge collapse = 14021
    \gray{14091} & \gray{Hybrid} & \gray{36f2c} & \gray{P} & \gray{Content} & \gray{OutE} & \gray{Summary hallucination (1) (=13971)}\\ \hline
    % Amish children killed, = 13971
    14092 & Abstractive & 36f2c & F & Additional & OthE & Attribution same topic but different location (2) \\ \hline
    % East Asian ivory anti-poaching education
    14049 & Abstractive & 36f2c & F & Semantic & PredE & Time shift led to inconsistent info (3)\\ \hline
    % Albarez decision - death or life in prison?
    14102 & Abstractive & 36f2c & F & Content & OutE & Summary hallucination (summary used ``the'' versus 1 of 4)\\ \hline
    \gray{14105} & \gray{Hybrid} & \gray{36f2c} & \gray{F} & \gray{Semantic} & \gray{PredE} & \gray{Time shift led to inconsistent info (2) (=14045)}\\ \hline
    % Iraqi reporter throws show at Pres Bush = 14045
    14108 & Abstractive & 36f2c & F & Additional & NE & Unclear why selected as refutation \\ \hline
    % Chinese computer virus arrest
    14115 & Hybrid  & 36f2c & F & Additional & OthE & Attributions contain related information (2,3)\\ \hline
    % Lack of sleep -> weight gain
  \end{tabular}
  %\parbox[b]{4.85in}{}
  \caption{TAC 2011: Machine Summaries: Task 2: 3 Attributing Sentences. L/Label: F=Full Support, P=Partial Support.}
  \label{tab:tac2011-machine-task2}
\end{table}


%%% CTI ANALYST MACHINE TASK 2 TABLE %%%
\begin{table}[h] \small
  %\parbox[b]{4.85in}{}
  \centering
  \begin{tabular}{|l|c|c|c|p{1.6cm}|p{1.1cm}|p{4.1cm}|}
    \hline
    \textbf{ID} & \textbf{Method} & \textbf{L} & \textbf{Annot.} &
    \textbf{Primary} & \textbf{2nd} & \textbf{Comment} \\
    \hline
    17040 & Abstractive & P & 73655 & Content  & OutE & Summary hallucination (=17160)\\ \hline
    % Inside TDrop2: Technical Analysis of new Dark Seoul Malware
    % Source document: (Stage 4) "It proceeds to randomly select an
    % executable file in the system32 folder, and performs process
    % hollowing against it."
    % Summary: In the fourth stage, the malware checked for parent processes
    % and performed process hollowing again.
    17041 & Abstractive & P & 73655 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution~1 (=17161)\\ \hline
    % Unit 42 has observed historical scans using IP addr shared by Volexity
    % All info in citation 1, 2/3 related
    17043 & Hybrid & P & 73655 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution~1\\ \hline
    % VirusTotal graph. All info in citation 1, 2/3 related.
    17044 & Hybrid & F & 73655 & Additional & OthE & Closely related information (2), related information (3), Summary $\approx$ Attribution~1\\ \hline
    % Certificate-based attack described.
    % Citation 1 is almost copy of summary sentence. Citation 2 describes vuln.
    17047 & Abstractive & P & 73655 & Additional & OthE & Related information (2)\\ \hline
    % Roshan_VC.iso, uses Brute Ratel C4 malware
    % (2) related info
    17048 & Abstractive & F & 73655 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution~1 \\ \hline
    % CVE-2022-26809
    % Citation 1 ~ summary
    17049 & Hybrid & P & 73655 & Semantic Additional & PredE OthE & Summary close to Attribution~1 but uses stronger language (``very likely'' versus ``likely''); Related information (2,3)\\ \hline
    % Iranian govt network compromise
    % Citation 1 ~ summary
    17053 & Abstractive & F & 73655 & Additional & OthE & Related information (3)\\ \hline
    % invest in awareness training, detection tool to reduce callback phish risk
    % citations 1 and 2 provide full support and additional information
    17056 & Hybrid & P & 73655 & Additional & OthE & Related information (3)\\ \hline
    % JsonWebToken patch information
    17057 & Abstractive & P & 73655 & Content & OutE & Summary contains info not present in attributions\\ \hline
    % list of products to detect and prevednt Conti ransomware, subset of list in citations (due to parsing?)
    17061 & Abstractive & P & 73655 & Additional & OthE & Related information (3) (=17181)\\ \hline
    % Iranian govt network compromise, related 17049
    % Summary: Playful Taurus continues to evolve its tactics...
    17063 & Hybrid & F & 73655 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution~1\\ \hline
    % VMWare advisory
    17065 & Hybrid & P & 73655 & Additional & NE & Unclear why selected as refutation\\ \hline
    % technical description malware 
    17066 & Abstractive & P & 73655 & Additional & OthE & Closely related information (2,3), Summary $\approx$ Attribution~1 \\ \hline
    % ML to detect network abuse
    17072 & Hybrid & F & 73655 & Additional & OthE & Closely related information (2), related information (3), Summary $\approx$ Attribution~1\\ \hline
    % AWS phishing attack
    17073 & Abstractive & P & 73655 & Semantic & EntE & Closely related information (2,3), Summary $\approx$ Attribution~1 but summary entity lacks sufficient information (``incidents'' versus ``incidents involving landing URLs'')\\ \hline
    % URL-based attack analysis
    17083 & Abstractive & P & 73655 & Additional & OthE & Closely related information (2,3), Summary $\approx$ Attribution~1\\ \hline
    % custom URI checksum to identify attack
    \gray{17160} & \gray{Abstractive} & \gray{N} & \gray{8f14c} & \gray{Content} & \gray{OutE} & \gray{Summary hallucination (=17040)}\\ \hline
    % 4th stage process hollowing
    \gray{17161} & \gray{Abstractive} & \gray{P} & \gray{8f14c} & \gray{Additional} & \gray{OthE} & \gray{Related information (2,3) (=17041)}\\ \hline
    % Unit 4 has observed historical scans targeting organizations using
    % IP addresses shared by Volexity
    \gray{17181} & \gray{Abstractive} & \gray{P} & \gray{8f14c} & \gray{Additional} & \gray{OthE} & \gray{Related information (3) (=17061)}\\ \hline
    % Playful Taurus, Iranian govt network compromise
  \end{tabular}
  %\parbox[b]{4.85in}{}
  \caption{Cyber Threat Intelligence: Machine Summaries: Analysts: Task 2: 3 Attributing Sentences. L/Label: F=Full Support, P=Partial Support, N=No Support.}
  \label{tab:cyber-machine-task2-analyst}
\end{table}


%%% CTI EXPERT MACHINE TASK 2 TABLE %%%
\begin{table}[h] \small
  %\parbox[b]{4.85in}{}
  \centering
  \begin{tabular}{|l|c|c|c|p{1.6cm}|p{1.1cm}|p{4.1cm}|}
    \hline
    \textbf{ID} & \textbf{Method} & \textbf{L} & \textbf{Annot.} &
    \textbf{Primary} & \textbf{2ndary} & \textbf{Comment} \\
    \hline
    16212 & Abstractive & P & 415f6 & Additional & OthE & Related information (3) (=17061, 17181)\\ \hline
    % Playful Taurus continues to evolve its tactics, and the analysis suggests that Iranian govt network have likely  been compromised.
    % Interesting -- in this case, it is likely, not very likely
    17592 & Hybrid & F & 5e2f7 & Semantic Additional & PredE OthE & Summary close to Attribution~1 but uses stronger language (``very likely'' versus ``likely''); Related information (2,3) (=17049) \\ \hline
    % Iranian network compromise
    17606 & Hybrid & F & 5e2f7 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution~1 (=17063) \\ \hline
    % advisory regarding 2 CVEs
    17633 & Abstractive & F & 84863 & Additional & NE & Unclear why selected as refutation  \\ \hline
    % summary attributes action to threat actor x4k, unclear why selected
    17639 & Abstractive & P & 84863 & Content & OutE & Summary hallucination \\ \hline
    % class object vuln
    % (2) hallucination: summary says vuln allows remote access class objects when (2) says the vuln is allows the search path of the system's class loader to be modified
    17642 & Hybrid & F & 84863 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution 1 \\ \hline
    % where downloaded file written
    % summary paraphrase of (1), (2,3) related info
    17643 & Abstractive & P & 84863 & Content Additional & OutE OthE & Summary contains information not in attributions, Related information (3) \\ \hline
    % OpenSSL suggested mitigations
    % (3) related
    % (2) missing entity: summary says OpenSSL suggests X, while the citation only suggests X without saying who suggested it
    17645 & Abstractive & P & 84863 & Content  & OutE & Summary hallucination (=17040, 17160) \\ \hline
    % confusion on malware stage
    17652 & Abstractive & N & 84863 & Additional & OthE & Related information (2) (=17047) \\ \hline
    % sample file associated with Brute Ratel C4
    % (2) related info, different sample file
    17658 & Abstractive & N & 84863 & Additional & OthE & Related information (3) (=17053) \\ \hline
    % mitigations for phishing
    17660 & Abstractive & P & 84863 & Content & OutE & Summary contains named entity while (3) uses pronoun \\ \hline
    % MS has provided mitigations & recs until a patch is released
    % missing entity: summary says MS provided mitigations but (3) uses "they"
    17661 & Hybrid & P & 84863 & Additional & OthE & Related information (3) (=17056) \\ \hline
    % JsonWebToken patch info
    17667 & Abstractive & F & 84863 & Content & GramE & Badly parsed attribution (2) \\ \hline
    % Auth0 team handled disclosure, patch
    % Summary paraphrase (1)
    % (2) had parsing issues of timeline so included several items but readable and relevant, list it as the objection
    % (3) provides supplemental info about the vuln
    17679 & Hybrid & F & 84863 & Additional & OthE & Related information (2,3) \\ \hline
    % summary approx (1)
    % (2,3) related
    17680 & Hybrid & F & 84863 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution~1 \\ \hline
    % summary paraphrase (1)
    % (2,3) related
    17684 & Hybrid & F & 84863 & Additional & OthE & Related information (2,3), Summary $\approx$ Attribution~1 \\ \hline
    % summary = (1)
    % (2,3) related
    17687 & Hybrid & F & 84863 & Additional & OthE & Related information (3) \\ \hline
    % URL requests similar to ProxyShell requests, reported by Mandiant
    % (3) related 
  \end{tabular}
  %\parbox[b]{4.85in}{}
  \caption{Cyber Threat Intelligence: Machine Summaries: Experts: Task 2: 3 Attributing Sentences. L/Label: F=Full Support, P=Partial Support, N=No Support.}
  \label{tab:cyber-machine-task2-expert}
\end{table}


%%% CRISISFACTS MACHINE TASK 2 TABLE %%%
\begin{table}[h] \small
  %\parbox[b]{4.85in}{}
  \centering
  \begin{tabular}{|l|c|c|c|p{1.6cm}|p{1.1cm}|p{4.1cm}|}
    \hline
    \textbf{ID} & \textbf{Method} & \textbf{L} & \textbf{Annot.} &
    \textbf{Primary} & \textbf{2nd} & \textbf{Comment} \\
    \hline
    17341 & Abstractive & P & 73655 & Content Additional & GramE OthE & Badly parsed, related information (2,3); Not enough information in summary to identify which fire\\ \hline
    % fire fought with planes and helicopters
    17344 & Abstractive & U & 73655 & Additional & OthE & Not enough information in summary to identify which disaster\\ \hline
    % generic: communities coming together in support
    17347 & Hybrid & F & 73655 & Semantic Additional & PredE OthE & Time shift led to inconsistent info (3); Attribution~2 for a different fire (=17467)\\ \hline
    % Holy fire burned 6200 acres, 5% contained
    % Citation 2 for Carr Fire, not Holy Fire
    17420 & Hybrid & P & 73555 & Semantic & PredE  & Time shift led to inconsistent info (3)\\ \hline
    % hurrican models trending west towards East Coast
    % summary says east coast, #3 says not known if east coast
    17425 & Abstractive & U & 73655 & Semantic Content & CircE GramE & Additional location information in summary inconsistent with attribution (2); Badly parsed attributions difficult to read (2,3)\\ \hline
    % red cross opened 2 new shelters
    17428 & Hybrid & F & 73655 & Semantic & PredE & Time shift led to inconsistent info (3), Summary $\approx$ Attribution~1 (=17488)\\ \hline
    % fire 200 acres -> 800 acres in one hour
    17429 & Hybrid & P & 73655 & Semantic & PredE & Time shift led to inconsistent info (3), Summary $\approx$ Attribution~1 (=17489)\\ \hline
    % Lilacfire burned 4100 acres, 60% contained, citation 3 says 90% contained
    17432 & Abstractive & P & 73655 & Content & OutE & Summary contains info not present in attributions\\ \hline
    % the storm is projected to potentially make landfall, prompted concerns + prep
    % no citations address concerns + prep
    17436 & Abstractive & N & 73655 & Additional & OthE & Attribution provided option not listed in summary (3)\\ \hline
    % consider evacuation plans
    % citation 3 has suggestion not in summary
    17439 & Hybrid & U & 73655 & Content Additional & OutE OthE  & Summary contains world knowledge not included in attribution (1); Attributions on related info (2,3)\\ \hline
    % 102h 12Z GFS model (Global Forecast System model)
    17448 & Abstractive & F & 73655 & Semantic & PredE & Time shift error led to inconsistent info (1,3)\\ \hline
    % fire fueled by strong Santa Ana winds, more favorable weather expected
    % citation 3 before more favorable weather predicted, citation 1 after
    17452 & Abstractive & F & 73655 & Additional & NE & Unclear why selected as refutation \\ \hline
    % localized flooding and power outages
    \gray{17467} & \gray{Hybrid} & \gray{F} & \gray{36f2c} & \gray{Semantic Additional} & \gray{PredE OthE} & \gray{Time shift led to inconsistent info (3); Attribution~2 for a different fire (=17347)}\\ \hline
    % the fire has burned 6200 acres and is currently 5% contained
    % Citation 2 for Carr Fire, not Holy Fire
    \gray{17488} & \gray{Hybrid} & \gray{F} & \gray{36f2c} & \gray{Semantic} & \gray{PredE} & \gray{Time shift led to inconsistent info (3) (=17428)}\\ \hline
    % fire 200 acres -> 800 acres in one hour
    \gray{17489} & \gray{Hybrid} & \gray{P} & \gray{36f2c} & \gray{Semantic} & \gray{PredE} & \gray{Time shift led to inconsistent info (3), Summary $\approx$ Attribution~1 (=17429)}\\ \hline
    % fire burned 4,100 acres and 60% contained, citation 3 says 90% contained
    17515 & Abstractive & F & 36f2c & Content & GramE & Badly parsed attribution (3)\\ \hline
    % Riverside and Shasta counties state of Emergency
  \end{tabular}
  %\parbox[b]{4.85in}{}
  \caption{CrisisFACTS: Machine Summaries: Task 2: 3 Attributing Sentences. L/Label: F=Full Support, P=Partial Support, N=No Support, U=Unclear.}
  \label{tab:crisisfacts-machine-task2}
\end{table}
